An Institution for Simple UML State Machines

We present an institution for UML state machines without hierarchical states. The interaction with UML class diagrams is handled via institutions for guards and actions, which provide dynamic components of states (such as valuations of attributes) but abstract away from details of class diagrams. We also study a notion of interleaving product, which captures the interaction of several state machines. The interleaving product construction is the basis for a semantics of composite structure diagrams, which can be used to specify the interaction of state machines. This work is part of a larger effort to build a framework for formal software development with UML, based on a heterogeneous approach using institutions.

==> preamble.tex <==
\usepackage{xspace,calc}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{times}
\usepackage[scaled=.85]{helvet}
\usepackage{babel}
\makeatletter\let\proof\@undefined\let\endproof\@undefined\makeatother%
\usepackage{amsmath,amssymb,amsthm,stmaryrd,mathrsfs}
\makeatletter\let\mathmargin\@mathmargin\makeatother
\usepackage{rotating}
\usepackage{xspace}
\usepackage{url}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{tikz}
\usetikzlibrary{matrix,shapes,arrows,calc}
\usetikzlibrary{backgrounds,fit}
\usepackage{enumitem}
\usepackage{float}
\usepackage{subfigure}
\usepackage{listings}
\lstset{%
  language=C,
  basicstyle=\ttfamily, %\fontsize{8pt}{8pt}\selectfont, % Standardschrift
  numbers=none,               % Ort der Zeilennummern
  numberstyle=\fontsize{6pt}{6pt}\selectfont,          % Stil der Zeilennummern
  %stepnumber=2,               % Abstand zwischen den Zeilennummern
  numbersep=7pt,              % Abstand der Nummern zum Text
  tabsize=4,                  % Groesse von Tabs
  extendedchars=true,         %
  breaklines=true,            % Zeilen werden Umgebrochen
  numberbychapter=false,
  %keywordstyle=\color{red},      
  %keywordstyle=[1]\textbf,    % Stil der Keywords
  %keywordstyle=[2]\textbf,    %
  %keywordstyle=[3]\textbf,    %
  %keywordstyle=[4]\textbf,   \sqrt{\sqrt{}} % 
  %stringstyle=\color{white}\ttfamily, % Farbe der String
  showspaces=false,           % Leerzeichen anzeigen ?
  showtabs=false,             % Tabs anzeigen ?
  captionpos=b,
  %frame=tb,
  xleftmargin=17pt,
  framexleftmargin=17pt,
  framexrightmargin=5pt,
  framexbottommargin=4pt,
  %backgroundcolor=\color{lightgray},
  showstringspaces=false,      % Leerzeichen in Strings anzeigen ?  
  escapeinside={(*@}{@*)},
  keywordsprefix={.},
}
% \usepackage[backend=biber,
%             style=llncs,
%             defernumbers=true,
%             firstinits=true,
%             maxnames=999,minnames=4,
%             isbn=false,doi=false,eprint=false]{biblatex}

\def\powerset{\wp}
\def\NZ{\mathbb{N}}
\def\ZZ{\mathbb{Z}}
\def\BZ{\mathbb{B}}
\def\RZ{\mathbb{R}}
\def\Rho{\mathit{P}}
\newcommand{\Eta}{H}
\newcommand{\Tau}{\mathit{T}}
\newcommand{\Ypsilon}{\mathit{Y}}
\newcommand{\omikron}{\ensuremath{o}}
\newcommand{\partialto}{\rightharpoonup}
\def\iff{\mathrel{\Leftrightarrow}}
\def\divop{\mathbin{\mathrm{div}}}
\def\modop{\mathbin{\mathrm{mod}}}
\def\im{\mathop{\mathrm{im}}}
\def\pll{\mathrel{\|}}
\def\fibop{\mathop{\mathrm{fib}}\nolimits}
\def\trueval{\mathit{tt}}
\def\falseval{\mathit{ff}}
\def\dom{\mathrm{dom}}
\def\infers{\mathrel{\vdash}}
\def\iteop{\mathrm{ite}}
\def\idop{\mathrm{id}}
\def\bottom{\bot}
\def\dbottom{\mathnormal{\bot\!\!\!\bot}}
\def\limp{\mathrel{\Rightarrow}}
\def\chooserel{\mathrel{\varepsilon}}
\def\lequiv{\mathrel{\Leftrightarrow}}
\def\partto{\mathrel{\rightharpoonup}}
\def\isorel{\mathrel{\cong}}
\def\sem#1{\mathopen\llbracket#1\mathclose\rrbracket}
\def\restrictop{\mathnormal{\upharpoonright}}
\def\preimop{{}^\bullet}
\def\compfun{\mathbin{\circ}}
\def\comprel{\mathbin{\circ}}
\def\isorel{\mathrel{\cong}}
\def\angleplus{\mathbin{\langle\!{+}\!\rangle}}
\def\fixop{\mathop{\smash{\mathbf{Y}}}\nolimits}
\def\applyop{\mathop{\mathrm{apply}}\nolimits}
\def\curryop{\mathop{\mathrm{curry}}\nolimits}
\newcommand{\structrule}[2]{\dfrac{%
\renewcommand{\arraystretch}{1.1}%
\begin{array}{@{}c@{}}#1\end{array}}{%
\renewcommand{\arraystretch}{1.1}%
\begin{array}{@{}l@{}}#2\end{array}}\vspace{3pt}}
\def\shows{\mathrel{\Vdash}}
\def\diverges{\mathnormal{\uparrow}}
\def\finop{\mathnormal{\mathscr{K}}}
\DeclareMathOperator{\colim}{\mathrm{colim}}
%\def\colim{\mathop{\mathrm{colim}}}
\def\invlim{\mathop{\underleftarrow{\lim}}}
\def\initdom{\emptyset_{\bottom}}
\def\xrightleftarrows#1#2{\mathrel{\raisebox{-.2ex}{$\begin{array}{@{}c@{}}\xrightarrow{#1}\\[-1.5ex]\xleftarrow[#2]{}\end{array}$}}}
\def\inclop{\hookrightarrow}

\def\IMP{{\textbf{IMP}}\xspace}
\def\syncat#1{{\normalfont\textrm{#1}}}
\def\semcat#1{{\normalfont\mathit{#1}}}
\newcommand{\code}[1]{\normalfont\texttt{\spaceskip=3pt\frenchspacing\def\{{\char123}\def\}{\char125}\def\^{\char94}\def\_{\char95}#1}}

\def\State{\Sigma}

\def\numsem#1{\mathop{\mathcal{N}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\boolsem#1{\mathop{\mathcal{B}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\arithsem#1{\mathop{\mathcal{A}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\nstrans{\mathrel{\rightarrow}}
\def\fvar{\mathop{\mathrm{fvar}}}
\def\floc{\mathop{\mathrm{fvar}}\nolimits_L}
\def\stateop{\mathop{\mathit{state}}}
\def\dvar{\mathop{\mathrm{dvar}}}
\def\updvarop{\mathop{\mathit{upd}}\nolimits_V}
\def\updprocop{\mathop{\mathit{upd}}\nolimits_P}
\def\newop{\mathop{\mathit{new}}}

\def\sostrans{\mathrel{\Rightarrow}}

\def\refsem#1{\mathop{\mathcal{R}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\stmsem#1{\mathop{\mathcal{S}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\contstmsem#1{\mathop{\mathcal{C}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\ASSN{{\textbf{ASSN}}\xspace}
\def\termsem#1{\mathop{\mathcal{T}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\frmsem#1{\mathop{\mathcal{F}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\phoare#1#2#3{\{ #1 \}\,#2\,\{ #3 \}}
\def\thoare#1#2#3{[ #1 ]\,#2\,[ #3 ]}
\def\flog{\mathop{\mathrm{flog}}}
\def\extop{\mathop{\mathrm{ext}}\nolimits}
\def\wpop{\mathop{\mathrm{wp}}\nolimits}
\def\wlpop{\mathop{\mathrm{wlp}}\nolimits}

% Literals
\newcommand{\clop}[1]{\syntax{\{}{#1}\syntax{\}}}

% Types
\newcommand{\ptop}[1]{\syntax{(}{#1}\syntax{)}}
\DeclareMathOperator{\typeop}{\mathit{type}}
\DeclareMathOperator{\baseop}{\mathit{base}}

% Type inference
\DeclareMathOperator{\fdop}{\mathit{fd}}
\newcommand{\entails}{\mathrel{\vdash}}
\newcommand{\annotated}{\mathrel{\triangleright}}

% Operational semantics
\DeclareMathOperator{\acttypeop}{\mathit{actual}}
\DeclareMathOperator{\flattenop}{\mathit{flatten}}
\DeclareMathOperator{\makeop}{\mathit{make}}
\DeclareMathOperator{\attrop}{\mathit{attr}}
\DeclareMathOperator{\methop}{\mathit{meth}}
\DeclareMathOperator{\implop}{\mathit{impl}}
\newcommand{\ordersrel}{\mathrel{\leadsto}}
\newcommand{\evalsto}{\mathrel{\downarrow}}

% Denotational semantics
\DeclareMathOperator{\evalop}{\mathit{eval}}
\DeclareMathOperator{\liftop}{\mathit{lift}}
\DeclareMathOperator{\oliftop}{\overline{\mathit{lift}}}
\DeclareMathOperator{\condop}{\mathit{cond}}
\DeclareMathOperator{\iterateop}{\mathit{iterate}}
\DeclareMathOperator{\sigop}{\mathit{sig}}

\newcommand{\Sig}[1]{\text{$#1$-$\mathrm{Sig}$}}
\newcommand{\Str}[1]{\text{$#1$-$\mathrm{Str}$}}
\newcommand{\trans}{\mathrel{\to}}
\def\reductop{\mathnormal{|}}
\def\natto{\mathrel{\dot{\mathnormal{\to}}}}

\newcommand{\opop}{\mathrm{op}}
\newcommand{\op}{^{\opop}}
\newcommand{\grothop}{\mathcal{G}}
\newcommand{\grothpair}[2]{\langle #1, #2\rangle}
\newcommand{\grothreduct}[3]{#1\reductop_{#2}#3}
\newcommand{\grothforward}[3]{#1^{\reductop_{#2}#3}}

\newcommand{\osSig}{\mathit{Sig}^{\leq}}
\newcommand{\osStr}{\mathit{Str}^{\leq}}
\newcommand{\osVal}{\mathit{\!Val}^{\leq}}
\newcommand{\osU}{U^{\leq}}
\newcommand{\osK}{\mathscr{T}^{\leq}}

\newcommand{\semtruth}{\mathnormal{\ast}}

%% UML
\newcommand{\uml}[1]{\textsf{#1}}
\newcommand{\stereotype}[1]{\uml{\flqq#1\frqq}}
\newcommand{\aggregation}{\raisebox{0.2pt}{\begin{sideways}\fontsize{6pt}{6pt}\selectfont$\lozenge$\end{sideways}}}
\newcommand{\composition}{\raisebox{0.2pt}{\begin{sideways}\fontsize{6pt}{6pt}\selectfont$\blacklozenge$\end{sideways}}}

\DeclareMathAlphabet{\mathsfsl}{OT1}{cmss}{m}{sl}

\newcommand{\FOL}{\text{\textit{FOL$^{=}$}}\xspace}
\newcommand{\PFOL}{\text{\textit{PFOL$^{=}$}}\xspace}
\newcommand{\PCFOL}{\text{\textit{PCFOL$^{=}$}}\xspace}
\newcommand{\SubPFOL}{\text{\textit{SubPFOL$^{=}$}}\xspace}
\newcommand{\SubPCFOL}{\text{\textit{SubPCFOL$^{=}$}}\xspace}
\newcommand{\ResSubPCFOL}{\text{\textit{ResSubPCFOL$^{=}$}}\xspace}

\newcommand{\angles}[1]{\langle #1 \rangle}


%% From MPhil
\newcommand{\category}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\functor}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\functorsymbol}[1]{#1}

\newcommand{\ModReduct}{\ensuremath{\category{Mod\_Reduct}}\xspace}

% These are institution functors
\newcommand{\Sen}{\functor{sen}}
\newcommand{\ModFunctor}{\functor{mod}}

% these are (projection) functions
%\newcommand{\Sig}{\ensuremath{\mathop{\text{\textbf{Sig}}}}}
\newcommand{\Mod}{\ensuremath{\mathop{\text{\textbf{Mod}}}}}
\newcommand{\Axioms}{\ensuremath{\mathop{\text{\textbf{Ax}}}}}
\newcommand{\flatten}{\ensuremath{\mathop{\text{\textit{flatten}}}}}
\newcommand{\LHS}{L.H.S\xspace}
\newcommand{\RHS}{R.H.S\xspace}
\newcommand{\Isabelle}{Isabelle\xspace}
\newcommand{\IsabelleHOL}{Isabelle/HOL\xspace}
\newcommand{\inj}{\mbox{\texttt{inj}}\xspace}
\newcommand{\pr}{\mbox{\texttt{pr}}\xspace}


%\usepackage{hetcasl}
%\usepackage{todonotes}


%% Names
\newcommand{\DB}{Dines Bj{\o}rner\xspace}
\newcommand{\Bjoerner}{Bj{\o}rner\xspace}

%% Languages
\newcommand{\COFI}{\textrm{\textsc{CoFI}}\xspace}
\newcommand{\CASL}{\textrm{\textsc{Casl}}\xspace}
\newcommand{\ModalCASL}{\textrm{\textsc{ModalCasl}}\xspace}
\newcommand{\RSL}{\textrm{\textsc{RSL}}\xspace}
\newcommand{\MiniDSL}{MiniDSL\xspace}

%% Tools
\newcommand{\Hets}{Hets\xspace}
\newcommand{\Spass}{SPASS\xspace}
\newcommand{\Vampire}{Vampire\xspace}

%% Institutions
\newcommand{\institution}[1]{\mathscr{#1}}
\newcommand{\instSigop}{\mathrm{Sig}}
\newcommand{\instSig}[1]{\instSigop^{\institution{#1}}}
\newcommand{\instModop}{\mathrm{Mod}}
\newcommand{\instMod}[1]{\instModop^{\institution{#1}}}
\newcommand{\instSenop}{\mathit{Sen}}
\newcommand{\instSen}[1]{\instSenop^{\institution{#1}}}
\newcommand{\instmodels}[2][]{\mathrel{\models^{\institution{#2}}_{#1}}}
\newcommand{\instPresop}{\mathrm{Pres}}
\newcommand{\instPres}[1]{\instPresop^{\institution{#1}}}

\newcommand{\ppinstitution}[1]{\institution{\powerset_{*}#1}}
\newcommand{\ppinstMod}[1]{\instMod{\ppinstitution{#1}}}
\newcommand{\ppinstmodels}[2][]{\instmodels[#1]{\ppinstitution{#2}}}

\newcommand{\ppmorphMod}[1]{\rho_{\institution{#1}, \ppinstitution{#1}}^{\instModop}}

\newcommand{\ippinstitution}[1]{\institution{\powerset_{*}^{\mathrm{i}}#1}}
\newcommand{\ippinstSig}[1]{\instSig{\ippinstitution{#1}}}
\newcommand{\ippinstSen}[1]{\instSen{\ippinstitution{#1}}}
\newcommand{\ippinstMod}[1]{\instMod{\ippinstitution{#1}}}
\newcommand{\ippinstmodels}[2][]{\instmodels[#1]{\ippinstitution{#2}}}

\newcommand{\ippinstcomorph}[1]{\mu^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphSig}[1]{\Phi^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphSen}[1]{\alpha^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphMod}[1]{\beta^{\ippinstitution{#1}, \institution{#1}}}

\newcommand{\incppinstitution}[1]{\institution{\powerset_{*}^{\hookrightarrow}#1}}
\newcommand{\incppinstSig}[1]{\instSig{\incppinstitution{#1}}}
\newcommand{\incppinstSen}[1]{\instSen{\incppinstitution{#1}}}
\newcommand{\incppinstMod}[1]{\instMod{\incppinstitution{#1}}}
\newcommand{\incppinstmodels}[2][]{\instmodels[#1]{\incppinstitution{#2}}}

\newcommand{\Val}{\mathrm{Val}}
\newcommand{\ENV}{\mathsf{Act}}
\newcommand{\SM}[1][]{\mathsf{SM}\text{$#1$}}

%\usepackage{xy}
%\xyoption{v2}
\newcommand{\xtrans}[4]{{#1}\xrightarrow[{#3}]{#2}{#4}}
\newcommand{\shorttrans}[4]{\xtrans{#1}{#2}{#3}{#4}}
\newcommand{\longtrans}[4]{\xtrans{#1}{#2}{#3}{#4}}
\newcommand{\llongtrans}[4]{\xtrans{#1}{#2}{#3}{#4}}
\newcommand{\lllongtrans}[4]{\xtrans{#1}{#2}{#3}{#4}}
\newcommand{\llllongtrans}[4]{\xtrans{#1}{#2}{#3}{#4}}
\newcommand{\emptyTrans}[1]{(\omega\reductop_{V_{\Eta_{#1}}}, \overline{e_{#1}} ,s_{#1})=(\omega'\reductop_{V_{\Eta_{#1}}}, \overline{e_{#1}},s_{#1}') \in (V_{\Eta_{#1}} \rightarrow \mathrm{Val}) \times \powerset(E_{\Sigma_{#1}}) \times S_{\Sigma_{#1}}}

%% Layout
%\parindent0pt
\allowdisplaybreaks
%\sloppy


